Numerical Methods for the 2-Hessian Elliptic Partial Differential Equation

The elliptic 2-Hessian equation is a fully nonlinear partial differential equation (PDE) that is related to intrinsic curvature for three dimensional manifolds. We introduce two numerical methods for this PDE: the first is provably convergent to the viscosity solution, and the second is more accurate, and convergent in practice but lacks a proof. The PDE is elliptic on a restricted set of functions: a convexity type constraint is needed for the ellipticity of the PDE operator. Solutions with both discretizations are obtained using Newton's method. Computational results are presented on a number of exact solutions which range in regularity from smooth to nondifferentiable and in shape from convex to non convex.

==> Two Hessian latex ArXiv/LatexCommands2Hessian.tex <==
% !TEX root = TwoHessian.tex

%----------------------------------------------{
% Packages and options
%----------------------------------------------
\usepackage[colorlinks, linkcolor=blue,  citecolor=blue, urlcolor=blue]{hyperref}%
\usepackage{url}
%----------------------------------------------
\usepackage{verbatim}
%\usepackage{showtags}
%\usepackage{showlabels}
%\usepackage{amsrefs}
%\usepackage[notref,notcite]{showkeys}
\usepackage{alltt}
%\usepackage{subfigure}
\usepackage{graphicx}
\graphicspath{{figures/}}
\usepackage{siunitx}
\usepackage{amsthm}

%%%%%%%%%%%%%%%%%%%%



% THEOREM Environments --------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
%\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
%\theoremstyle{remark}
\newtheorem{remark}{Remark}[section]
\theoremstyle{definition}
\newtheorem{example}{Example}[section]


%%%%%%%%%%%%%%%%%%%%
%  Basic Commands
%%%%%%%%%%%%%%%%%%%%
%----------------------------------------------
% norms, absolute value
\newcommand{\norm}[1]{\Vert#1\Vert}
\newcommand{\Norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\vert#1\vert}
\newcommand{\Abs}[1]{\left\vert#1\right\vert}

%% Basic Commands
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\median}{median}
\DeclareMathOperator{\dv}{div}
\newcommand{\grad}{\nabla}
\newcommand{\bq}{\begin{equation}}
\newcommand{\eq}{\end{equation}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
%\newcommand{\dm}{d}
\newcommand{\Rd}{\R^d}
\newcommand{\Rn}{\R^n}
\newcommand{\e}{\epsilon}
\newcommand{\bO}{\mathcal{O}}
\newcommand{\Lip}{Lipschitz}
%% Sectioning Commands
\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}


%% For this paper
\newcommand{\lam}{\lambda}
\newcommand{\sig}{\sigma_2}
\newcommand{\sigex}{\bar \sigma}
\DeclareMathOperator{\sort}{sort}
\DeclareMathOperator{\diag}{diag}
\newcommand{\x}{\textbf{x}}

%%% Finite Differences 
\newcommand{\dt}{\rho}
\newcommand{\dx}{h}
\newcommand{\Sk}{{F}}
\newcommand{\Mp}{S_\rho}
\newcommand{\Dxx}{\mathcal{D}_{xx}}
\newcommand{\Dyy}{\mathcal{D}_{yy}}
\newcommand{\Dzz}{\mathcal{D}_{zz}}
\newcommand{\Dxy}{\mathcal{D}_{xy}}
\newcommand{\Dxz}{\mathcal{D}_{xz}}
\newcommand{\Dyz}{\mathcal{D}_{yz}}
\newcommand{\Dt}{\mathcal{D}}

%% Laplacians
\newcommand{\IL}{\Delta_\infty}
\newcommand{\pLap}{\Delta_p}
\newcommand{\Lap}{\Delta}
\newcommand{\MC}{\Delta_1}
\newcommand{\ME}{\lambda_1}
\newcommand{\grhs}{g}
